Uncertainty-Aware Multi-Expert Knowledge Distillation for Imbalanced Disease Grading

Automatic disease image grading is a significant application of artificial intelligence for healthcare, enabling faster and more accurate patient assessments. However, domain shifts, which are exacerbated by data imbalance, introduce bias into the model, posing deployment difficulties in clinical applications. To address the problem, we propose a novel \textbf{U}ncertainty-aware \textbf{M}ulti-experts \textbf{K}nowledge \textbf{D}istillation (UMKD) framework to transfer knowledge from multiple expert models to a single student model. Specifically, to extract discriminative features, UMKD decouples task-agnostic and task-specific features with shallow and compact feature alignment in the feature space. At the output space, an uncertainty-aware decoupled distillation (UDD) mechanism dynamically adjusts knowledge transfer weights based on expert model uncertainties, ensuring robust and reliable distillation. Additionally, UMKD also tackles the problems of model architecture heterogeneity and distribution discrepancies between source and target domains, which are inadequately tackled by previous KD approaches. Extensive experiments on histology prostate grading (\textit{SICAPv2}) and fundus image grading (\textit{APTOS}) demonstrate that UMKD achieves a new state-of-the-art in both source-imbalanced and target-imbalanced scenarios, offering a robust and practical solution for real-world disease image grading.

==> tabs/imbalanced_kd_eyepacs.tex <==
\begin{table*}[tp!]
\caption{Performance on EyePacs dataset of individually trained ResNet models (Top), feature-based KD models (Middle), and logits-based KD models (Bottom). 
% The best results are highlighted in bold. Suboptimal results are indicated with an underscore. 
} 
%Performance of our proposed D-Persona framework and several public methods for multi-rater medical image segmentation on the public LIDC-IDRI dataset. We show the results of individually trained U-Net models (\ie, using annotations from a single expert, Top), generation-based methods (with different sampling numbers, Middle), and personalized segmentation works (Bottom), respectively.
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cccc|cccc}
\toprule[1.5pt]
\multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Sources-imbalanced KD (\%)}  & \multicolumn{4}{c}{Targets-imbalanced KD (\%)} \\
\cline{2-9} &  OA$\uparrow$&  mAcc$\uparrow$ &  F1 $\uparrow$ &  MAE $\downarrow$ &  OA$\uparrow$&  mAcc$\uparrow$ &  F1 $\uparrow$ &  MAE$\downarrow$       \\ \midrule
Resnet50 ($Exp_1$) &81.10 & 51.10 & 77.32 & 0.3425 
& 64.59 & 51.94 & 60.90 & 0.5623 \\
Resnet50 ($Exp_2$) & 80.98 &51.75 & 77.47 & 0.3515 &64.25 & 51.80 & 60.84 & 0.5697 \\
Resnet18 ($Sup$) & 61.90 & 49.66 & 58.49 & 0.5851 
&80.22 & 51.82 & 76.58 & 0.3640 \\\midrule
FitNet~\cite{romero2014fitnets} & 56.81 & 35.37 &49.31 & 0.7944   & 75.85 & 32.06 &68.35 &0.5313  \\

%Prob. U-Net (\#10) &0.2181 &88.79 &88.60 &88.43 & \multicolumn{5}{c}{\multirow{7}{*}{N/A}}  \\
%Prob. U-Net (\#30) &0.2169 &88.79 &88.80 &88.73 & & & & & \\
%Prob. U-Net (\#50) &0.2168 &88.80 &88.87 &88.81 & & & & & \\
%D-Persona (\uppercase\expandafter{\romannumeral1}, \#10) &0.1461 &90.24 &90.75 &90.51 & & & & & \\
%D-Persona (\uppercase\expandafter{\romannumeral1}, \#30) &0.1375 &90.42 &91.23 &91.16 & & & & & \\
RKD~\cite{park2019relational} &66.09 &\underline{49.04} &61.25 &0.5839  &\textbf{81.30} &48.42 &77.41 &\textbf{0.3996} \\
% \rowcolor{lm_purple_low} ProSeg (prior \#50) &\textbf{0.1077} &\textbf{91.62} &\textbf{91.46}&\textbf{91.43} & & & & & \\ 
\midrule

KD~\cite{HintonVD15} &65.25 & 47.32 & 59.72 &0.5752 
& \underline{81.25} & 50.76 & \textbf{77.85} & 0.4314  \\
DKD~\cite{zhao2022decoupled}  & 65.03 & 43.90 & 58.34 & \underline{0.5736} 
& 80.65 &\underline{51.08} &77.41 &0.4473  \\
SDD ~\cite{wei2024scaled}  & \underline{66.75} & 47.51 & \underline{61.87} & 0.5758 
& 81.07 &50.28 &77.25 &0.4117  \\
% Pionono &0.1502 &90.00 &90.10 &88.97 &87.94 &89.11 &89.55 &88.76 &88.84 \\
% UMKD (\uppercase\expandafter{\romannumeral2}) &0.1444 &90.31 &90.38&89.17&88.54&89.50&90.03 &88.60 &89.17  \\
\rowcolor{lm_purple_low} UMKD & \textbf{67.84} & \textbf{51.26} & \textbf{64.04} &\textbf{0.5604} 
& 81.18 & \textbf{51.54} &\underline{77.41}& \underline{0.4098} \\
\midrule
\rowcolor{lm_purple_low}\textbf{$\triangle$} 
&\textcolor{green!50!black}{+1.09} 
&\textcolor{green!50!black}{+3.75} 
&\textcolor{green!50!black}{+2.17} 
&\textcolor{green!50!black}{+0.0154} 
&\textcolor{green!50!black}{+0.11} 
&\textcolor{green!50!black}{+1.26} 
&\textcolor{green!50!black}{+0.16} 
&\textcolor{green!50!black}{+0.0019} \\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab_eyepacs}
\vspace{-1em}
\end{table*}
